RegMiner: Towards Constructing a Large Regression Dataset from Code Evolution History

Bug datasets consisting of real-world bugs are important artifacts for researchers and programmers, which lay empirical and experimental foundation for various SE/PL research such as fault localization, software testing, and program repair. All known state-of-the-art datasets are constructed manually, which inevitably limits their scalability, representativeness, and the support for the emerging data-driven research. In this work, we propose an approach to automate the process of harvesting replicable regression bugs from the code evolutionary history. We focus on regression bug dataset, as they (1) manifest how a bug is introduced and fixed (as normal bugs), (2) support regression bug analysis, and (3) incorporate a much stronger specification (i.e., the original passing version) for general bug analysis. Technically, we address an information retrieval problem on code evolution history. Given a code repository, we search for regressions where a test can pass a regression-fixing commit, fail a regressioninducing commit, and pass a working commit. In this work, we address the challenges of (1) identifying potential regression-fixing commits from the code evolution history, (2) migrating the test and its code dependencies over the history, and (3) minimizing the compilation overhead during the regression search. We build our tool, RegMiner, which harvested 537 regressions over 66 projects for 3 weeks, created the largest replicable regression dataset within shortest period, to the best of our knowledge. Moreover, our empirical study on our regression dataset shows a gap between the popular regression fault localization techniques (e.g, delta-debugging) and the real fix, revealing new data-driven research opportunities.

==> change-example.tex <==
if(...){
  TagMacher tags = tagCache.get(projectName).match(...);
  <@\textcolor{red}{- filterTagsSeparately ? filter(getAllRefs()).values() : rs.values();}@>
  <@\textcolor{blue}{+ filterTagsSeparately ? filter(refs)).values() : rs.values();}@>
  
  for(...){...}
}




==> definitions.tex <==
%\section{Definitions}\label{sec:def}
%In this section, we present the details of our approach. For simplicity, we assume that the program under test is in the form of a method and the goal is to achieve maximum branch coverage of an individual method.
%This work targets for branch coverage of individual method.

We first define the terminology. We call the method under test the \textbf{target method}, denoted as $m_t$.
%In section, we first formally define several definitions across the whole article.
%\begin{newdef}\label{def:flag_method}
%\textbf{Flag Method}.
We refer to a method $m$ as a called method if $m$ is called directly in the target method $m_t$ or indirectly through a called method.
A called method $m$ is called a \textbf{flag method} if there exists a condition $c$ of a branching node in the target method $m_t$ which directly or indirectly depends on the value returned by $m$.
In addition, we call \textit{that} boolean value used in the condition $c$ an \textbf{interprocedural flag} and the branch to be covered an \textbf{interprocedural flag branch}.
%\end{newdef}
For example, method \texttt{check\-Pre\-condi\-tion()} in Listing~\ref{lst:example_main} is a flag method of the target method \texttt{get()}.
Given a test case $t\leftarrow$\texttt{keys=[0, 1], value=-20}, there are two uncovered interprocedural flag branches in \texttt{get()} method, i.e., branch $\langle 2, 3\rangle$ and branch $\langle 5, 6\rangle$.
The corresponding interprocedural flags are the values returned by method \texttt{check\-Pre\-con\-di\-tion()} and by method \texttt{checkValue()}.

Furthermore, given an interprocedural flag branch $b$ which depends on a flag method $m$, there may be multiple program paths in $m$ which return a boolean value such that $b$ is covered.
We call such program paths in $m$ as the \textbf{required paths} for covering $b$.
We call the last branch in a required path as the \textbf{required branch}.
For example, for branch $\langle 2, 3\rangle$ in Listing~\ref{lst:example_main},
the path $\langle 2, 3, 4\rangle$ in Listing~\ref{lst:example_precondition} is a required path,
and the branch $\langle 3, 4\rangle$ is a required branch.

%\begin{newdef}\label{def:anchor_branch}
%\textbf{Required Flag Branch.}
%Given that there is an uncovered branch $b$ in the target method $m_t$, it depends on an interprocedural flag $f$ returned from a flag method $m$.
%Let $Exit$ be the set of direct branches reaching exits of the CFG of $m$, we define \textbf{required flag branch} as a set of branches $R\subseteq Exit$ so that executing a branch $r\in R$ can cover $b$.
%\end{newdef}

%In this work, the required flag branches serve as ``anchor'' and we use their branch distances to aggregate a continuous value for the corresponding interprocedural flag branch.


==> empirical-study.tex <==
\section{Empirical Study}\label{sec:empirical-study}
Based on the regression dataset we construct in Section~\ref{sec:evaluation},
we investigate the following empirical research questions:
\begin{itemize}[leftmargin=*]
  \item \textbf{ERQ1.} What do the regression-inducing commits do?
  \item \textbf{ERQ2.} How likely a regression can be fixed by reverting the regression-inducing changes in practice?
  %\item \textbf{ERQ3.} How is the performance of state-of-the-art regression localization technique such as delta-debugging?
  \item \textbf{ERQ3.} What are the follow-up potential research opportunities?
\end{itemize}

\subsection{Study Design}\label{sec:empirical-study-design}
\subsubsection{Semantic Analysis}
In this study, we investigate the general semantics of changes made in regression-inducing commits. %in quantitative and qualitative manner.
%For quantitative analysis, we check the amount of changes made in two types of commits in different granularity.
Specifically, we generate rough semantic labels for each commits
in three types of labels, i.e., refactoring, feature enhancement, and bug-fixing for a commit.
We let a commit have multiple semantic labels.

Given a commit $c$ consisting of a set of hunks $H$.
A hunk $h\in H$ is a sequence of added or deleted lines, denoted as $h = \langle Add, Del \rangle$
where $Add$ represents the set of added lines and $Del$ represents the set of deleted lines.
Moreover, we use the function $code(.)$ to have the code body of either part of a hunk.
For example, $code(h.Add)$ represents the code body of the added code in hunk $h$.
Also, we use $|code(.)|$ to represent the length of the code body.
We attach the semantic label with the following rules:
\begin{itemize}[leftmargin=*]
  \item \textbf{Refactoring}:
    We regard a commit to have a refactoring label if $\exists h_i\in H, h_j\in H$ ($h_i \neq h_j$), so that
    \begin{enumerate}
      \item Either $code(h_i.Add)$ is similar to $code(h_j.Del)$ or vice versa, and
      \item $|code(h_i.Add)|$ (or $|code(h_i.Del)|$) should be larger than a threshold $th_{len_r}$.
    \end{enumerate}
    Intuitively, it means that a piece of code is moved to another location in the project.
    Without losing generality, we use $code(h_i.Add)$ and $code(h_j.Del)$ to illustrate similarity calculation.
    Specifically, the similarity is calculated as $\frac{2\times |LCS(code(h_i.Add), code(h_j.Del))}{min(|code(h_i.Add)|, |code(h_j.Del)|)}$ where $LCS(., .)$
    is the longest common subsequence between two pieces of code.
    If the similarity is above a threshold $th_{sim}$, we consider a refactoring happens.
  \item \textbf{Feature Enhancement}:
    We regard a commit to have a feature enhancement label if
    \begin{enumerate}
      \item $\exists h_i \in H$, so that
        \begin{enumerate}
          \item Either $|code(h_i.Del)| = 0$ or $\frac{|code(h_i.Add)|}{|code(h_i.Del)|} > th_{r}$. Here $th_{r}$ is a user-defined threshold to measure the size difference between added and deleted code, and
          \item $code(h_i.Add)$ is larger than the threshold $th_{len_f}$, and
          \item $\nexists h_j\in H$ so that $code(h_i.Add)$ is similar to $code(h_j.Del)$.
        \end{enumerate}
        or,
      \item $\frac{\sum_{i} |code(h_i.Add)|}{\sum_{j} |code(h_j.Del)| + \epsilon} > th_{ar}$ and $\sum_{i} |code(h_i.Add)|$ should be larger than the threshold $th_{len_f}$.
      Here, $h_i$ and $h_j$ should not be refactoring hunks.
      Overall, the ratio of the length of accumulated addition over that of accumulated deletion should be larger than a threshold $th_{ar}$.
    \end{enumerate}

    Intuitively, we require that we have a hunk which includes a large number of non-refactoring additions.
  \item \textbf{Bug Fixing}:
    We regard a commit to have a bug fixing label if the message of $c$ include keywords as ``fix'' and ``bug''.
    Typically, we cannot infer the bug fixing semantics without any specifications.
    With limited information, we use commit message as the only reference to infer the bug fixing label.
\end{itemize}

\subsubsection{Revert Analysis}
Reverting the change back to the past, is the fundamental rationale of the most influential regression debugging technique -- delta debugging \cite{kiss2018hddr, misherghi2006hdd, zelleryesterday, wang2021probablisitic, brummayer2009fuzzing}.
In this study, we investigate how far we can infer a regression fix,
assuming that delta-debugging can successfully recommend a failure-inducing change.
Given a regression-fixing commit has change set $H_f$ and its corresponding regression-inducing commit has change set $H_i$,
we first define the notation $same\_location(h_i, h_j)$ (where $h_i \in H_f$ and $h_j \in H_i$).
Specifically, $same\_location(h_i, h_j)$ return true if
(1) the method $m_i$ where $h_i$ happens in the regression-fixing revision can be re-identified to the method $m_j$ where $h_j$ happens in the regression-inducing revision, and
(2) the relative location of $h_i$ in $m_i$ can overlap with that of $h_j$ in $m_j$.
Readers can refer to Section~\ref{sec:code-reidentification} for how we re-identify code elements across the history.
Then, we conduct the following analysis for our empirical questions:
\begin{itemize}[leftmargin=*]
  \item \textbf{Revert Analysis:}
    We consider the fix of a regression adopt change revert if $\exists h_i\in H_f, h_j\in H_i$ so that
    \begin{enumerate}
      \item either $code(h_i.Add)$ is similar to $code(h_j.Del)$ or $code(h_i.Del)$ is similar to $code(h_j.Add)$, and
      \item $same\_location(h_i, h_j)$ is true.
    \end{enumerate}
  \item \textbf{Estimated Distance to Fix:}
    Given $h_i\in H_f, h_j \in H_i$, we categorize the distance of regression fix change from the regression-inducing change $cat_d(h_i, h_j)$ as:
    \begin{enumerate}
      \item \textbf{Level 0}: the method where $h_i$ happens can be re-identified to the method where $h_j$ happens, $code(h_i)$ relatively overlaps with $code(h_j)$.
      \item \textbf{Level 1}: the method where $h_i$ happens can be re-identified to the method where $h_j$ happens, but $code(h_i)$ does not relatively overlap with $code(h_j)$.
      \item \textbf{Level 2}: the file where $h_i$ happens can be re-identified to the file where $h_j$ happens.
      \item \textbf{Level 3}: the file where $h_i$ happens cannot be re-identified to the file where $h_j$ happens.
    \end{enumerate}
    Here, we measure the minimum $cat_d(h_i, h_j)$ for each regression,
    indicating the most optimistic estimation on how close a fix is to the regression-inducing change.
\end{itemize}

Note that, we do not run a specific delta-debugging algorithm.
Instead, we assume the theoretically best performance of delta-debugging to return the failure-inducing change,
and observe how it can leads to a final fix solution.

\subsubsection{Runtime Configuration}\label{sec:runtime-configuration}
In this study, we choose
the threshold of changed length for refactoring $th_{len_r}=5$,
the threshold of code similarity $th_{sim}=0.8$,
the threshold of the accumulated length for feature enhancement $th_{ar}=15$, and
the threshold of changed length for feature enhancement $th_{len_f}=10$.

\subsection{Study Results}\label{sec:empirical-study-result}
\subsubsection{Results (ERQ1): }\label{sec:erq1}
\autoref{fig:ric-label} shows the distribution of regression-inducing commits on different semantic labels.
Overall, the regression-fixing commits are almost evenly distributed in the three semantic labels (i.e., 29.1\% for bug fixing, 30.9\% for refactoring, and 19.7\% for feature enhancement).
Moreover, we cannot attach any labels on 231 regression-fixing commits.
The major reason is that regression-fixing commits can involve huge number of deletions,
which can hardly fit in the three categories.
Thus, we regard the semantic of those commits as unknown.
%While feature enhancement takes the majority (\linyun{?\%}),
%linyun{?\%} of the regressions are incurred during refactoring and \linyun{?\%} are incurred during bug fixing.
Moreover, an individual regression-inducing commit can serve very diverse purposes.
We observe that 106 commits share at least two labels, and 9 commits share all three labels.

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.16]{image/venn.jpg}
  \caption{Semantic labels of regression-inducing commits}
  \label{fig:ric-label}
\end{figure}

Not like normal bugs where a specification can be described by only a limited number of test cases,
regression bugs have a working revision serving as the specification which allows us to derive abundant test cases to guard the program behaviors.
Therefore, we deem that an automatic solution to decide 
\textit{
when regression test generation is required can be practical remedy to prevent regression bugs incurred by refactoring, bug fixing, and feature enhancement.
}


\subsubsection{Results (ERQ2): }\label{sec:erq2}
Our studies show that 26 (i.e., 4.8\%) of regressions can be fixed by reverting the change applied in the corresponding regression-inducing commit.
Moreover, \autoref{fig:fix-distance} shows the distribution of the estimated distance-level from the regression-fixing location to the regression-incurring location.
Note that, we apply an over-estimation analysis in this study,
the real-world distribution can lean towards high-level distance.

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.22]{image/fix-distance.pdf}
  \caption{Optimistic distance from a regression fix to its failure-inducing location}
  \label{fig:fix-distance}
  %\vspace{-10pt}

\end{figure}

We find that, even with such an optimistic estimation, there are still 33.5\% of the regressions have level 2 and level 3 distance.
It indicates that,
with a single test case (which is a practical assumption in real-world development scenarios),
even a perfect delta-debugging technique in theory,
there is still a non-trivial gap between the location (and change) it reports and where to fix in such regressions.
Typically, an automated repair technique consists of a fault localization technique and a repair technique.
Our results suggest that a \textit{fix localization} problem is non-trivial,
which should be addressed to lay a solid foundation for regression-pair technique.

\subsubsection{Results (ERQ3): }\label{sec:erq3}
Our empirical studies reveal abundant research opportunities, such as
\begin{itemize}[leftmargin=*]
  \item Which task (e.g., refactoring or bug fixing) needs the protection of regression test generation?
  \item Whether the fix of a regression just needs a revert?
  \item Can we predict a fix localization solution for a regression?
\end{itemize}

With traditional program analysis technique,
those questions can only be addressed with heuristics or project-specific insights.
In contrast, \tool can continuously collect large regression dataset and further provide data-driven facilities for their remedies.
Our dataset is available at \cite{regminer}.

%\subsubsection{Results (ERQ4): }\label{sec:erq4}

\begin{comment}
\begin{lstfloat}[t]
\lstinputlisting[caption={Target method under test, containing two interprocedural flags.}, label={lst:example_main}]{example_main.tex}
\end{lstfloat}

\begin{lstfloat}[t!]
\lstinputlisting[caption={Precondition checking code, which is called by the target method and produces a boolean flag.},
label={lst:example_precondition}]{example_precondition.tex}
\end{lstfloat}

\begin{lstfloat}[t!]
\lstinputlisting[caption={Key comparison code, which is called by the target method and produces a boolean flag.},
label={lst:example_contain}]{example_contain.tex}
\vspace{-5pt}
\end{lstfloat}

\end{comment}

\subsection{Threats to Validity}
This study has two internal threats and one external threat.
First, we have rough estimation of semantic labels, which may not be 100\% accurate in practice.
For example, the semantic label of feature enhancement are estimated as large code additions.
Some bug-fixing may also require to add much code.
Second, when investigating the distance of regression fix to the regression introduction,
we apply optimistic estimation.
%Despite it does not influence our conclusion,
A more precise measurement is required to further the future investigation.
The external threat lies in that our empirical results depend on a set of user-defined thresholds (see Section~\ref{sec:runtime-configuration}).
We select those threshold based on our expertise and experience in academic and industry.
In the future work, we will adjust more sets of thresholds and adapt more accurate solutions to generalize our conclusion.


==> exp-design.tex <==
\subsection{Experiment Design}
\subsubsection{Close-world Experiment}
We evaluate \tool in the close-world experiment regarding precision and recall.
Note that, this work is essentially an information-retrieval task on code evolutionary history.
In this study, we manually collect \gtNum regression-fixing commits and \gtNum non-regression fixing commits
from Github repositories for the measurement of precision and recall.
The scale of our ground-truth regression dataset is larger than the regression datasets used in various regression studies.
%(see \autoref{fig:other-regression-number}).
To avoid bias, we construct the regression benchmark without any help of \tool.
Specifically, we search for closed Github issues each of which uniquely mentions a commit as its solution.
Then, we filter those issues based on its labels and description.
We prioritize the issues with labels as ``regression'' or ``bug'', or with description with the keyword of ``regression''.
Then, we confirm the real regressions by manually checking the evolution history for regression-inducing commits, and migrating the test cases.
As a result, we confirmed \gtNum regressions from 23 Java projects by this means (see \cite{regminer} for more details).
By similar means, we identified \gtNum non-regression bugs.
%\autoref{tab:ground-truth} shows the overview of our ground truth regressions.
%Moreover, to evaluate we select \gtNum non-regression bug-fixing commits.

We apply \tool on all the regression and non-regression fixing commits to measure the precision and recall.
Let the number of true regressions be $N$ ($N=50$), the number of reported regressions be $M$, and the number of reported true regressions be $K$,
the precision is $\frac{K}{M}$, the recall is $\frac{K}{N}$.
%Given different machine have the runtime overhead different,
%we evaluate the efficiency by the number of revisions each solution needs to visit.
\two{
We choose the empirical regression-inducing probability $p$ as 0.05.
}

\begin{comment}
\begin{table}[t]
\small
\centering
\caption{The overview of manually collected regressions on Github}
\label{tab:ground-truth}
\begin{tabular}{|l|c|c|c|c|}
\hline
\textbf{Project Name} & \textbf{Size} & \textbf{\#Commits} & \textbf{Duration} & \textbf{\#Regression} \\ \hline
XXX                   & 500K          & 10K                & 10 years          & 5                     \\ \hline
XXX                   & 500K          & 10K                & 10 years          & 5                     \\ \hline
XXX                   & 500K          & 10K                & 10 years          & 5                     \\ \hline
\end{tabular}
\end{table}
\end{comment}

\subsubsection{Open-world Experiment}
\tool is designed to mine regressions from Git repositories with zero human intervention.
In this experiment, we collect Git repositories from Github and run \tool to mine regressions for \weekNum weeks.
We evaluate \tool regarding the authenticity and the diversity of
the mined regressions in both quantitative and qualitative manner.

\paragraph{Quantitative Analysis}
We quantitatively estimate how likely the tested feature in the regression-fixing revision (RFC) exists in the regression-inducing revision (RIC),
based on the rationale that the feature in RFC is very likely to be preserved in RIC
if the test covers similar set of code elements in both revisions.
Specifically, for each mined regression $reg = \langle rfc, ric, t \rangle$,
we run $t$ against \textit{rfc} and \textit{ric} to have their covered method set $E_{rfc}$ and $E_{ric}$.
%Here, $E_{rfc}$ and $E_{ric}$ are the set of methods.
We consider $m_f \in E_{rfc}$ can be aligned with $m_i \in E_{ric}$ if UMLDiff algorithm ~\cite{xing2005umldiff} can match them.
Therefore, we measure the feature coverage similarity in \textit{rfc} and \textit{ric} by:
$$
sim_f(reg) = \frac{|E_{rfc} \cap E_{ric}|}{min(|E_{rfc}|, |E_{ric}|)}
$$

%Therefore, we can have the distribution of syntactic feature similarity of all mined regressions.

\paragraph{Qualitative Analysis}
%Note that, RFC may undergo huge refactoring from RIC, which makes UMLDiff fail.
%We classify the regressions regarding their syntactic feature similarity into three categories, i.e., small (0-0.33), medium (0.33-0.66), and large (0.66-1.0).
%We further choose 30 regressions with the lowest coverage similarity for qualitative analysis.
We further sample 30 regressions with high coverage score (>0.9), 30 with medium score (0.4-0.7), and 30 with low score (<0.1).
To facilitate the manual investigation, we build a tool to visualize and compare revision difference, run test cases against each revision, and revert changes between revisions.
A screenshot of the tool is available at our anonymous website \cite{regminer}.
We recruit two graduate students (both with over 5 years of Java programming experience) to manually verify each regression based on the following template questions:
\begin{itemize}[leftmargin=*]
  \item What is the feature RFC aims to fix?
  \item What is the reason of the bug?
  \item Why can the feature work well before RIC?
\end{itemize}
The two students were asked to write down their answer independently.
Then, they are further asked to discuss with each other to reconcile their answers.
Given a regression, if they agree that the feature tested in RFC is different from the feature tested in RIC,
we conclude the regression is a false positive.

\paragraph{Diversity Analysis}
We measure the diversity of the regression dataset by investigating the diversity of
(1) topics of used libraries of the regression and
(2) the exception types of each bug.
Assume the regressions are distributed in $K$ library topics\footnote{We follow the topic categories defined in maven central repository (i.e., \url{https://mvnrepository.com/repos/central}), e.g., core utilities, collection, JSON libraries, etc.}, and reported in $L$ exception types (e.g., \texttt{NullPointerException}),
we compare the diversity between our collected datasets and Defects4j on
(1) the number of library topics and reported exception types, and
(2) the information entropy of bug distribution on the topics and exception types.

\subsubsection{Ablation Study}
%To the best of our knowledge, \tool is the first technique to retrieve runnable regressions in the code repository.
In the study, we disable and enable the three components respectively to evaluate their effectiveness.

\paragraph{Regression Potential}
%As for regression fixing commit prediction, the size of ground truth regression set is too small to provide convincing results.
%We run \tool on \prjNum Github repositories for \weekNum weeks and collect the reported regressions for this study.
Assuming that the number of regression fixing commits is $N$ ($N=$\regressionNum), we randomly select another $N$ bug fixing commits.
Then, we let \tool generate regression potential metric for each fixing commit,
comparing the metrics distribution of the two groups.
\one{
Moreover, we evaluate our regression potential metrics by investigating the effectiveness of its rank on the regression-fixing commits.
Specifically, given $N$ regression-fixing commits and $\alpha N$ ($\alpha > 1$) non-regression fixing commits, we evaluate how many regression-fixing commits
can \tool report by looking the first $k$\% reported commits.
Given that non-regression fixing commits are usually more frequent than regression-fixing commits, 
we choose $\alpha=2$ in this study.
}

\paragraph{Test Dependency Migration and Validation Effort Minimization}
In this study, we disable the capability of test dependency migration and validation effort minimization separately.

\one{
\begin{itemize}[leftmargin=*]
  \item \textbf{Disabled Test Dependency Migration (\tool$_{\neg TDM}$):}
    We have \tool$_{\neg TDM}$ for \tool with test dependency migration disabled.
    In \tool$_{\neg TDM}$, we copy the identified test case into the target revision without dependency analysis.
  \item \textbf{Simplified Validation Effort Minimization (\tool\\$_{\neg VEM+bisec}$):}
    We have \tool$_{\neg VEM+bisec}$ for \tool with validation effort minimization simplified.
    In \tool$_{\neg VEM+bisec}$, we search for regressions by using git-bisect strategy \cite{git-bisect}.
    Moreover, if \tool$_{\neg VEM+bisec}$ visits a revision $c_{inv}$ without any feedback, we conservatively estimate a failure feedback on $c_{inv}$.
  \item \textbf{Disabled TDM and Simplified VEM (\tool$_{\neg TDM}$ + $bisect)$:}
    We have \tool$_{\neg TDM}$ + $bisect)$ for \tool with test dependency migration disabled and search for regression with git-bisect strategy.
  \item \textbf{Disabled TDM and Simplified VEM (\tool$_{\neg TDM}$ + \\$gitblame$):}
    We have \tool$_{\neg TDM}$ + $gitblame)$ for \tool with test dependency migration disabled and search for regression with git-blame strategy on the difference between \textit{rfc} and \textit{rfc}-1.
    We consider the strategy on a regression successful if 
    (1) git-blame can report \textit{ric} and
    (2) the test migration from \textit{rfc} to \textit{ric} is successful.
\end{itemize}
}





%In \tool$_{\neg VEM+all}$, we search for regressions by iteratively checking each commit from the regression-fixing commit to the initial commit.
%It stops either when a regression-inducing commit is found or the initial commit is reached.



We compare \tool with the aforementioned variants on the datasets in both close-world and open-world experiments.
Given the open-world experiment takes \weekNum weeks
in this study, we replicate the experiment with the following simplification.
Given \tool reports $N$ regressions in the open-world experiment ($N=$\regressionNum in this study),
we randomly sample $2\times N$ bug-fixing commits, and
run \tool, \tool$_{\neg TDM}$, and \tool$_{\neg VEM}$ on the $3\times N$ bug fixing commits to
observe their performance.


%\subsubsection{Regression Potential Evaluation and Retrieval}


%\subsubsection{Regression Retrieval}
%We collect \linyun{?} Github repositories, as the input of \tool.
%We run \tool on those repositories for 3 weeks (limited by paper submission deadline),
%and observe how many regressions \tool can report.


==> good_example.tex <==
public boolean accept(File f)
  {
    if (f.isDirectory()) {
      return true;
    }
    String suffixe = null;
    String s = f.getName();
    int i = s.lastIndexOf('.');
    if ((i > 0) && (i < s.length() - 1)) {
      suffixe = s.substring(i + 1).toLowerCase();
    }
    return (suffixe != null) && (appartient(suffixe));
  }
  
boolean appartient(String suffixe)
  {
    for (int i = 0; i < this.lesSuffixes.length; i++) {
      if (suffixe.equals(this.lesSuffixes[i])) {
        return true;
      }
    }
    return false;
  }

==> hard_example3.tex <==
public static boolean equals(Object o1, Object o2){
 if(o1==null){
    return o2==null;
 }
 return o1.equals(o2);
}

==> implementation.tex <==
\section{Implementation}\label{sec:implementation}
We build our implementation \tool (Evosuite on Interprocedural Flag Problem) sitting on \evo~\cite{Fraser:2011:EAT:2025113.2025179}.
To this end, we modify its instrumentation and extend the fitness functions of by \texttt{fbranch} fitness.
The demo and tutorial is accessible at~\cite{evoipf}.


==> intro0.tex <==
\section*{Extended Abstract}
\subsection*{1. Problem}
% the important of bug repository
Bug datasets are fundamental infrastructure to support various software engineering researches
such as software testing, and bug repair.
%The effectiveness of a new proposed research methodology (e.g., on bug prediction, localization, repair, etc.),
%usually needs to be verified on a set of collected bugs in an experiment.
The SE/PL community has taken decades to construct bug datasets,
and finally gravitate to the state-of-the-art dataset, Defects4j~\cite{just2014defects4j}, taking seven years to collect over 800 bugs.

% the difficulty of constructing a bug repository
While bug datasets like Defects4j \cite{just2014defects4j} and CoREBench \cite{bohme2014corebench} have made significant contribution to the community,
there are still concerns that their sizes are relatively small (and, thus arguably less representative \cite{sobreira2018dissection}),
regarding
(1) their diversity (e.g., bug types of concurrency, API misuse, non-deterministic, etc.) and
(2) the needs of applying the emerging data-driven and AI techniques in SE tasks.
However, comparing to the cost of labelling an image or a sentence in the AI community,
manually collecting and labelling a bug is far more expensive.
It requires to
(1) prepare at least two versions of code project (i.e., a correct version and a buggy version),
(2) set up at least one test case passing the correct version and failing the buggy version, and
(3) isolate an environment where the bug can be well replicated.

% existing work of constructing a bug repository
Existing bug datasets are usually constructed manually,
which naturally limits its scalability.
A recent work, BugBuilder \cite{jiang2021extracting}, is proposed to isolate bug-fixing changes in a bug-fixing revision.
Applied on many code repositories,
BugBuilder can potentially generate a bug dataset similar to Defects4j, with a much larger size.
In such a bug dataset,
the buggy code is labelled with their fixes, potentially facilitating various data-driven bug-related learning tasks.
%each bug has a fixing version (i.e., the bug-fixing revision), a buggy version (i.e., the revision before the bug-fixing revision), and a test case passing the former and failing the latter.

% why a regression bug repository
In this work, we further propose an approach, \tool, to harvest \textit{regression bugs} from the code repository.
Regression bugs are bugs which make an existing working function (or feature) fail.
Comparing to a non-regression bug dataset collected by BugBuilder,
an ultra-large regression repository has the following two benefits.


%\lstinputlisting[caption={
%A Branch Relevant to Object States
%}, label={lst:change-example}, float=h]{change-example.tex}

% reason: more referenced specification for learning tasks
\noindent\textbf{(1) Less Specification-missing Problem:}
%To support data-driven bug-related tasks,
%regression dataset suffers less from the speci\-fi\-cation-missing problem, comparing to a non-regression bug dataset.
Software bugs are essentially the inconsistencies between the implementation and its specification.
Thus, a bug-related solution such as debugging and repair can be less reliable without sufficient specification as the input.
%Note that, non-regression bug datasets only have their buggy code annotated with the fixes,
%in addition to a few test cases to sanity-check the passing version.
%Therefore, it is arguably effective to design a bug-related learning task (e.g., fix prediction) from even a very large dataset.
%However, a fix on the code is basically the consequence of code editing (e.g., change an operator from \texttt{>} to \texttt{>=}), which embeds limited \textit{specification} information to learn.
%Therefore, it is arguably effective to design a bug-related learning task (e.g., fix prediction) from even a very large bug dataset.
%consisting of the buggy code with their labelled fixes.
In contrast to non-regression bug dataset where each bug is manifested with a few failing test cases,
regression bugs are additionally equipped with their past passing version as a much stronger referenced specification,
providing a more informative semantics to
explain why the bug happens, and
potentially facilitating the recommendation of their fixes.
In addition, they also provide a special way for us to
detailedly investigate how the code implementation begins to deviate from the expected program behavior.
%(2) construct or train data-driven solutions for tasks like software debugging and repair.

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.2]{image/other-regression-number.pdf}
  \caption{The distribution of the number of regressions used in 14 regression localization work from 1999 to 2021 in SE/PL community (See details in \cite{regminer}).
  }\label{fig:other-regression-number}
  \vspace{-10pt}
\end{figure}

% reason: target for regression analysis
\noindent\textbf{(2) Scalable Benchmark for Regression Analysis:}
From the perspective of benchmark construction, a large regression dataset can lay foundation for various regression analysis.
Existing regression analysis works (e.g., regression localization) are usually evaluated with limited number of regressions,
given that their collection is highly laborious.
\autoref{fig:other-regression-number} shows the distribution of the number of real-world regressions used in 15 research works from the year of 1999 to 2021
\cite{yi2015synergistic, wang2019explaining, zelleryesterday, buhse2019vedebug, tan2015relifix, pastore2013radar, cohen2015localization, khalilian2021cgenprog, zhang2012faulttracer, yu2012towards1, yu2012towards2, brummayer2009fuzzing, yu2012practical, artho2011iterative}.
Overall, the mean number of regressions is 16.6, and the median is 12.5.
Even worse, different benchmarks are used in different work,
making it difficult to compare their performance.
A large-scale benchmark can not only mitigate this issue,
but support various systematic empirical studies on regressions.


% our solution
\subsection*{2. Approach}
In this work, we design \tool to automate the regression harvesting process with \textit{zero} human intervention.
\tool can
continuously harvest a large number of replicable regression bugs from code repositories (e.g., Github).
Technically, we address an information retrieval problem in the context of software evolution history,
i.e., retrieving runnable regressions on a code repository.
Our approach takes a set of code repositories (e.g., Git) as input, and
isolates a set of regressions with their running/replicable environment as output.
Specifically, we construct a regression by searching in code repositories for
a regression-fixing commit denoted as $rfc$,
a regression-inducing commit denoted as $ric$,
a working commit (before $ric$) denoted as $wc$, and
a test case denoted as $t$
so that $t$ can pass $rfc$ and $wc$, and fail $ric$.
To this end, we first design a measurement to select those bug-fixing commits with more regression potential.
%Then, we rank BFCs with their quantified RFC potential in descent order.
Next, for each such potential regression-fixing commit, $rfc$,
we further search for a test case $t$ which can pass $rfc$,
fail the commit before (denoted as $rfc-1$), and pass a commit further before $rfc-1$.
Our search process addresses the technical challenges of
\begin{itemize}[leftmargin=*]
  \item \textbf{Regression Potential}: identifying relevant code changes in $rfc$ to migrate through the code evolution history.
  \item \textbf{Test Case Migration}: adopting the library upgrades with the history.
  \item \textbf{Validation Effort Minimization}: minimizing the compilation overhead and handling incompilable revisions
\end{itemize}


\begin{comment}
\begin{itemize}[leftmargin=*]
  \item \textbf{Relevant Change Identification: }
    The search process needs to migrate the test case $test$ and its dependencies from $rfc$ to the commits before without any compilation errors.
    However, the changes applied by a bug-fixing commit can contains
    (1) the added code depended by the test case $test$,
    (2) bug-fixing change, and
    (3) irrelevant changes to the bug.
    We need to only migrate the first type of changes because the second type of changes can make the $test$ pass in $rfc-1$ while the third type of changes can cause unnecessary compilation errors (see an example in Section~\ref{sec:motivating-example}).
    Thus, how to identify the first type of changes?
  \item \textbf{Library Adaption: }
    A regression can last for years, during which the depended libraries by the project can go through a series of upgrades.
    How can we detect such library upgrades and what is the solution to adapt to such upgrades?
  \item \textbf{Compilation Overhead Minimization: }
    Checking out and compiling every commit in a code repository is time-consuming.
    Moreover, some revisions are inherently in-compilable.
    How can we speed up the search process for more regression regarding the in-compilable revisions?
\end{itemize}
\end{comment}

%In this work, we propose a systematic change inference approach to address the above challenges.
%Our approach adopts a \checks{customized delta-debugging} between $rfc$ and $rfc-1$ to slice the minimized set of changes for migration;
%detects version-related compilation errors and transforms the test case $test$ according to the specific version; and
%conducts a novel binary search on the commit history regarding the compilation-error reversion.

% results
\subsection*{3. Evaluation}
We build \tool to mine Java regressions, supporting maven and gradle projects in current implementation.
We evaluate \tool with the following research questions,
more details of our experiment are available at our anonymous website \cite{regminer}.
\begin{itemize}[leftmargin=*]
  \item \textbf{RQ1 (Close-world Experiment):} Whether \tool can mine regressions from Git repositories accurately and completely?
  \item \textbf{RQ2 (Open-world Experiment):} Whether \tool can continuously mine authentic regressions from real-world Git repositories? How diverse is our constructed regression dataset?
  %\item \textbf{RQ3 (Authenticity Evaluation):} How authentic the mined regressions in the field?
  \item \textbf{RQ3 (Ablation Study):} How each component in \tool,
    i.e., regression potential estimation, test dependency migration, and validation effort minimization,
    contribute to the mining effectiveness and efficiency?
  %\item \textbf{RQ3:} What is the runtime overhead of \tool?
  %\item \textbf{RQ4:} How effective are our technical contributions to discover regressions (i.e., ablation study)?
  %\item \textbf{RQ3:} How is the runtime overhead of \tool?
\end{itemize}


\subsubsection*{3.1 Results (RQ1): Close-world Experiment}
We evaluate \tool in the close-world experiment regarding precision and recall.
%Note that, this work is essentially an information-retrieval task on code evolutionary history.
In this study, we manually collect \gtNum regression-fixing commits and \gtNum non-regression fixing commits
from Github repositories for the measurement of precision and recall.
The scale of our ground-truth regression dataset is much larger than the regression datasets used in various regression studies
(see \autoref{fig:other-regression-number}).
To avoid bias, we construct the regression benchmark without any help of \tool.
Specifically, we search for closed Github issues each of which uniquely mentions a commit as its solution.
Then, we filter those issues based on its labels and description.
We prioritize the issues with labels as ``regression'' or ``bug'', or with description with the keyword of ``regression''.
Then, we confirm the real regressions by manually checking the evolution history for regression-inducing commits, and migrating the test cases.
As a result, we confirmed \gtNum regressions from 23 Java projects by this means (see \cite{regminer} for more details).
By similar means, we identified \gtNum non-regression bugs.
%\autoref{tab:ground-truth} shows the overview of our ground truth regressions.
%Moreover, to evaluate we select \gtNum non-regression bug-fixing commits.

We apply \tool on all the regression and non-regression fixing commits to measure the precision and recall.
Let the number of true regressions to be $N$ ($N=50$), the number of reported regressions to be $M$, and the number of reported true regressions to be $K$,
the precision is $\frac{K}{M}$, the recall is $\frac{K}{N}$.
Overall, we achieve 100\% precision and 56\% recall in the experiment.

\subsubsection*{3.2 Results (RQ2): Open-world Experiment}
\tool is designed to mine regressions from Git repositories with zero human intervention.
In this experiment, we collect Git repositories from Github and run \tool to mine regressions for \weekNum weeks.
We evaluate \tool regarding the authenticity and the diversity of
the mined regressions in both quantitative and qualitative manner.

Overall, \tool construct a regression dataset consisting of \regressionNum regressions over the \prjNum projects within \weekNum weeks.

%\autoref{fig:coverage-distribution} shows the distribution of feature coverage similarity of all the mined regressions.
%We can see that the most regressions have a high feature coverage similarity (mean is 0.85),
%indicating that the most regression features tested in the regression-inducing commit are likely preserved in the regression-fixing commit.
%
%\begin{figure}
%  \centering
%  \includegraphics[scale=0.25]{image/coverage-distribution.pdf}
%  \caption{Feature Coverage Similarity Distribution}\label{fig:coverage-distribution}
%\end{figure}

%We confirm that 89 out of 90 regressions (each one third for high, medium, and low coverage similarity score) are authentic.
%%\linyun{The 3 false positives comes from the reported regressions with medium and low coverage score}.
%We observe that the authentic regressions with low coverage score are usually caused by
%(1) code refactoring and
%(2) deviated program execution leading to the coverage of new extra code.
%As for the latter, the bug leads the program to execute other branches and, in turn, invoke new code,
%causing a large $E_{ric}$ including many utility functions.
%Nevertheless, in most cases, the core feature is still within $E_{rfc} \cap E_{ric}$.

\subsubsection*{3.3 Results (RQ3): Ablation Study}
In the study, we disable and enable the function of test case migration and validation effort minimization respectively to evaluate their effectiveness.
\autoref{tab:performance} shows that the overall regression retrieval performance.
Overall, comparing to the baselines, our solutions shows their effectiveness.
While achieving the leading performance,

\begin{table}[h]
\caption{The overall performance of regression retrieval}
\label{tab:performance}
\small
\tabcolsep=0.1cm
\centering
\begin{tabular}{|l|ccc|cc|}
\hline
\multirow{2}{*}{\textbf{Approach}} & \multicolumn{3}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Close-world \\ Experiment\end{tabular}}} & \multicolumn{2}{l|}{\textbf{\begin{tabular}[c]{@{}l@{}}Open-world \\ Experiment\end{tabular}}} \\ \cline{2-6}
                                   & \multicolumn{1}{c|}{\textbf{Prec}}   & \multicolumn{1}{l|}{\textbf{Rec}}   & \textbf{Time (h)}  & \multicolumn{1}{l|}{\textbf{\#Reg}}                     & \textbf{Time (h)}                    \\ \hline
RegMiner                           & \multicolumn{1}{c|}{1.0}             & \multicolumn{1}{c|}{0.56}           & 4.29               & \multicolumn{1}{c|}{1035}                               & 135.38                               \\ \hline
RegMiner$_{\neg TDM}$              & \multicolumn{1}{c|}{1.0}             & \multicolumn{1}{c|}{0.32}           & 2.21               & \multicolumn{1}{c|}{604}                                & 64.29                                \\ \hline
RegMiner$_{\neg VEM+biset}$        & \multicolumn{1}{c|}{1.0}             & \multicolumn{1}{c|}{0.47}           & 2.74               & \multicolumn{1}{c|}{629}                                & 73.84                                \\ \hline
\end{tabular}
\end{table}




%In conclusion, we summarize our contributions as follows:
%\begin{itemize}[leftmargin=*]
%  \item We propose a fully automated regression mining technique,
%    which allows us to continuously harvest regressions from a set of code repositories with zero human intervention.
%  \item We build our \tool tool with extensive experiments evaluating its precision and recall to mine regressions.
%    The results show that \tool is accurate, effective, and efficient to mine regressions from code repositories.
%  \item We construct a regression dataset with \tool within \weekNum weeks. We foresee that the size of our regression dataset can keep growing with time,
%      opening the a number of research opportunities on bug analysis.
%  %\item We conduct an empirical study on the regression dataset, showing the limitation of delta-debugging techniques for regression analysis, and revealing a number of research opportunities which can be facilitated by data-driven solutions in the future.
%\end{itemize}

% paper structure
\begin{comment}
The rest of the paper is structured as follows.
Section~\ref{sec:motivating-example} presents our motivating example to illustrate technical challenges.
Section~\ref{sec:approach} describes our approach in detail.
Section~\ref{sec:evaluation} evaluates the effectiveness of our approach.
Section~\ref{sec:empirical-study} presents our empirical study.
Section~\ref{sec:related_work} reviews related work.
Section~\ref{sec:conclusion} discusses related issues and concludes the paper.
\end{comment}


==> limitation_branch_distance.tex <==
public AxisSpace reserveSpace(Graphics2D g2, ...){
  if(!isVisible()){...}
}

boolean isVisible(){
  return this.visible;
}

==> limitation_environment_construction.tex <==
void eConnect(...){
  ...
  if(isConnected()){...}
}

boolean isConnected(){
    return (this.m_socket != null)
        && (this.m_socket.isConnected())
        && (!this.m_socket.isClosed());
} 

==> limitation_mutation_type.tex <==
boolean reverseArcMakesSense(BayesNet bayesNet, int head, int tail){
  ...
  if (!isArc(bayesNet, head, tail)) {
    return false;
  }
}

boolean isArc(BayesNet bayesNet, int head, int tail){
  for(int iParent = 0; iParent < bayesNet.getParentSet(head).getNrOfParents(); iParent++) {
    if(bayesNet.getParentSet(head).getParent(iParent) == tail)
      return true;
  return false;
}

==> limitation_normal_parent.tex <==
boolean getMethod(String p1, String p2){
  ...
  if (p1.equals(p2)
    && signatureCorrect(p1)) {
    return false;
  }
}

==> limitation_trivial_flag.tex <==
public void solvePhase1(final SimplexTableau tableau) throws OptimizationException {
 ...
  if (!MathUtils.equals(tableau.getRhs(), 0, this.epsilon)) {
    throw new NoFeasibleSolutionException();
  }
}

public static boolean equals(double x, double y, double eps) {
  return equals(x, y) || FastMath.abs(y - x) <= eps;
}

==> motivating-example.tex <==
%\section{Challenges and Example}
%The first and third challenges is straightforward to understand,
%we provide a motivating example to further illustrate the challenges of test case migration.
\autoref{tab:motivating-example} shows more details of challenges of test case migration,
which shows a regression-fixing commit extracted from the Commons Lang project under Apache\footnote{See issue description in https://issues.apache.org/jira/browse/LANG-818.}.
The regression lasts for 17 months and spans \linyun{?} commits.
Even confirmed as a RFC with a usable regression-relevant test case,
migrating the test case to the regression-inducing commit requires address the following questions.

%\begin{comment}
\noindent\textbf{- What changes in a bug-fixing commit to migrate?}
In practice, a bug-fixing commit can include multiple changes.
Some changes are fix-relevant, and some may not.
Migrating fixing changes into the past commits can cause the test case pass the buggy revisions.
The changes in regression-fixing commit involve two Java files and one XML file.
The change semantics include
regression fix (line 4-18 in \texttt{FastDateFormater.java} and line 2 in \texttt{changes.xml}),
feature enhancement (line 2 in \texttt{Fast\-Date\-Formater\-.java})
and (ir)relevant test case creation (\texttt{Fast\-Date\-Formater\-Test\-.java}).
In this case, the regression fix can involve both the Java source code and configuration file.
Migrating the changes in XML file makes us fail to confirm this commit $c$ is a BFC
because the test case can pass both $c$ and $c-1$.
%\end{comment}

\noindent\textbf{- What code in a bug-fixing revision to migrate?}
In order to search for a regression, we need to determine a test case and migrate it across the evolution history.
However, the project has undergone huge changes between the regression-introducing revision and the regression-fixing revision.
Specifically, the changes include \linyun{?} files, \linyun{methods}, and \linyun{?} lines of source code.
On one hand, miss migrating the test depended code can cause compilation errors.
On the other hand, migrating irrelevant can introduce additional risks of compilation errors in the regression-introducing revision.

\noindent\textbf{- How to adapt the libraries used in the past?}
Even if we identify the correct subsets of changes and code to migrate along with the test case,
the migrated code still need adaption in the regression-introducing revision.
In this case, the JDK library version used in the regression-introducing revision is 1.5, which is much lower than that used in the regression-fixing revision,
which incurs compilation errors.
JDK 1.5 does not support \texttt{@Override} annotation for methods overriding Java interface methods,
which makes some migrated code incompilable.
Moreover, some fields in the regression-fixing revision need to be further modified with \textit{static} to avoid compilation errors.

\begin{table}
\caption{A regression fix commit consisting of 39 additions and 6 deletions in Apache Common Lang project.}
\label{tab:motivating-example}
\small
\begin{tabular}{| p{7.8cm} | }
%\multicolumn{2}{c}{Regression Fix Commit} & \multicolumn{2}{c}{Regression Introducing Commit}\\
%\hline
%\textbf{File} & \textbf{Fixed Version}  &  \textbf{Pre-Fix Version}\\
\hline
.../chan\-ges.xml
\begin{lstlisting}
<action>...</action>
<@\textcolor{blue}{+ <action>FastDateFormat's ...</action>}@>
<action>...</action>
\end{lstlisting} \\
\hline\hline
.../Fast\-Date\-For\-mater.java
\begin{lstlisting}
...
<@\textcolor{blue}{+ Math.max(mStandard.length(), mDaylight.length());}@>
...
<@\textcolor{red}{- mTimeZone = timeZone;}@>
<@\textcolor{blue}{+ mLocale = locale;}@>
<@\textcolor{blue}{+ mStyle = style;}@>
...
@Override
public void appendTo(StringBuffer buffer, Calendar calendar) {
    <@\textcolor{red}{- if(mTimeZone.useDaylightTime() ...) \{ }@>
    <@\textcolor{red}{-     buffer.append(mDaylight);}@>
    <@\textcolor{blue}{+ TimeZone zone = calendar.getTimeZone();}@>
    <@\textcolor{blue}{+ if (zone.useDaylightTime() ...)}@>
    <@\textcolor{blue}{+ buffer.append(getTimeZoneDisplay(zone, true, mStyle, mLocale));}@>
    } else
        <@\textcolor{red}{- buffer.append(mStandard);}@>
        <@\textcolor{blue}{+ buffer.append(getTimeZoneDisplay(zone, false, mStyle, mLocale));}@>
}
...
\end{lstlisting}\\
\hline\hline
.../Fast\-Date\-Printer\-Test.java
\begin{lstlisting}
...
<@\textcolor{blue}{+ import static org.junit.Assert.assertNotNull;}@>
...
<@\textcolor{blue}{+ @Test}@>
<@\textcolor{blue}{+ public void testCalendarTimezoneRespected()\{}@>
<@\textcolor{blue}{+ ...}@>
<@\textcolor{blue}{+ FormatCache.getPatternForStyle(dateStyle, null, locale);}@>
<@\textcolor{blue}{+ String actualValue = FastDateFormat.getInstance(pattern).format(cal);}@>
<@\textcolor{blue}{+ assertEquals(expectedValue, actualValue);}@>
<@\textcolor{blue}{+ \}}@>
\end{lstlisting}\\
\hline
\end{tabular}
\end{table}

In this work, we design \tool to
(1) predict which bug-fixing commit is with more regression potential,
(2) migrate test case with both static and dynamic dependency analysis, and
(3) design a history travel algorithm to further reduce the number of revision to be investigated.
As for the test case migration, \tool can accurately generate a differencing class dependency graph between the regression-fixing revision and the regression-introducing revision, as showed in \autoref{fig:motivating-example}.
Specifically, starting with the test cases to be migrated,
we apply both static and dynamic analysis to slice the relevant program elements (e.g., class, interface, method, etc.) in the regression-fixing revision to migrate.
\autoref{fig:motivating-example} shows that there are only a limited number of program elements are involved,
comparing to the \linyun{?} changed files and \linyun{?} changed methods.
Each identified migrating elements will be annotated as a change type such as addition (the \texttt{+} sign) and modification (the \texttt{?} sign),
which can guide the migration in the regression-introducing revision.

\begin{figure}[t]
  \centering
  \includegraphics[scale=0.56]{image/example.pdf}
  \caption{Differencing Class Dependency Graph to Guide the Test Migration}\label{fig:motivating-example}
\end{figure}



==> seed-example.tex <==
public int example(String a, int b){
    int x1 = a.length() + b;
    if(x1==123){...} //branch distance is sufficient
    if(x1==1234567890){...} //seed can improve test efficiency
    boolean x2 = b > 987654321;
    if(x2){...} //seed can improve test efficiency
    String x3 = a.substring(0, 6);
    String x4 = a.substring(7, a.length());
    if(x3.equals(x4)){...} //seed cannot improve test efficiency
} 

==> unfair_example.tex <==
public void setLocation(String string)
    throws NumberFormatException
  {
    if (isISO6709(string)) {
      parseISO6709(string);
    } else {
      parseString(string);
    }
  }

private boolean isISO6709(String check)
  {
    return ((check.startsWith("+")) || (check.startsWith("-"))) && (check.endsWith("/"));
  }
